Diffstar: A Fully Parametric Physical Model for Galaxy Assembly History

We present Diffstar, a smooth parametric model for the in-situ star formation history (SFH) of galaxies. Diffstar is distinct from conventional SFH models that are used to interpret the spectral energy distribution (SED) of an observed galaxy, because our model is parametrized directly in terms of basic features of galaxy formation physics. The Diffstar model assumes that star formation is fueled by the accretion of gas into the dark matter halo of the galaxy, and at the foundation of Diffstar is a parametric model for halo mass assembly, Diffmah. We include parametrized ingredients for the fraction of accreted gas that is eventually transformed into stars, $\epsilon_{\rm ms},$ and for the timescale over which this transformation occurs, $\tau_{\rm cons};$ some galaxies in Diffstar experience a quenching event at time $t_{\rm q},$ and may subsequently experience rejuvenated star formation. We fit the SFHs of galaxies predicted by the IllustrisTNG (TNG) and UniverseMachine (UM) simulations with the Diffstar parameterization, and show that our model is sufficiently flexible to describe the average stellar mass histories of galaxies in both simulations with an accuracy of $\sim0.1$ dex across most of cosmic time. We use Diffstar to compare TNG to UM in common physical terms, finding that: (i) star formation in UM is less efficient and burstier relative to TNG; (ii) galaxies in UM have longer gas consumption timescales, $\tau_{\rm cons}$, relative to TNG; (iii) rejuvenated star formation is ubiquitous in UM, whereas quenched TNG galaxies rarely experience sustained rejuvenation; and (iv) in both simulations, the distributions of $\epsilon_{\rm ms}$, $\tau_{\rm cons}$, and $t_{\rm q}$ share a common characteristic dependence upon halo mass, and present significant correlations with halo assembly history. [Abridged]

==> abstract_mnras.tex <==
\begin{abstract}
We present \dstar, a smooth parametric model for the in-situ star formation history (SFH) of galaxies. The \dstar model is distinct from traditional SFH models because it is parametrized directly in terms of basic features of galaxy formation physics. \dstar includes ingredients for: the halo mass assembly history; the accretion of gas into the dark matter halo; the fraction of gas that is eventually transformed into stars, $\mseff$; the timescale over which this transformation occurs, $\taucons$; and the possibility that some galaxies will experience a quenching event at time $\qtime$, and may subsequently experience rejuvenated star formation. We show that our model is sufficiently flexible to describe the average stellar mass histories of galaxies in both the \tng (TNG) and \um (UM) simulations with an accuracy of $\sim$0.1 dex across most of cosmic time. We use \dstar to compare TNG to UM in common physical terms, finding that: (i) star formation in UM is less efficient and burstier relative to TNG; (ii) UM galaxies have longer gas consumption timescales, relative to TNG; (iii) rejuvenated star formation is ubiquitous in UM, whereas quenched TNG galaxies rarely experience sustained rejuvenation; and (iv) in both simulations, the distributions of $\mseff$, $\taucons$, and $\qtime$ share a common characteristic dependence upon halo mass, and present significant correlations with halo assembly history. We conclude with a discussion of how \dstar can be used in future applications to fit the SEDs of individual observed galaxies, as well as in forward-modeling applications that populate cosmological simulations with synthetic galaxies.
\end{abstract}

